Systematic human learning and generalization from a brief tutorial with explanatory feedback

Neural networks have long been used to model human intelligence, capturing elements of behavior and cognition, and their neural basis. Recent advancements in deep learning have enabled neural network models to reach and even surpass human levels of intelligence in many respects, yet unlike humans, their ability to learn new tasks quickly remains a challenge. People can reason not only in familiar domains, but can also rapidly learn to reason through novel problems and situations, raising the question of how well modern neural network models capture human intelligence and in which ways they diverge. In this work, we explore this gap by investigating human adults' ability to learn an abstract reasoning task based on Sudoku from a brief instructional tutorial with explanatory feedback for incorrect responses using a narrow range of training examples. We find that participants who master the task do so within a small number of trials and generalize well to puzzles outside of the training range. We also find that most of those who master the task can describe a valid solution strategy, and such participants perform better on transfer puzzles than those whose strategy descriptions are vague or incomplete. Interestingly, fewer than half of our human participants were successful in acquiring a valid solution strategy, and this ability is associated with high school mathematics education. We consider the challenges these findings pose for building computational models that capture all aspects of our findings and point toward a possible role for learning to engage in explanation-based reasoning to support rapid learning and generalization.

==> titlepage.tex <==
\begin{titlepage}

    \vspace*{7.5cm}

    \begin{center}
        {\huge
        Systematic human learning and generalization from 
        
        a brief tutorial with explanatory feedback}
        
        {\large Andrew J. Nam$^{1*}$, James L. McClelland$^1$}
    \end{center}
   
    \vfill
    $^1$ Department of Psychology, Stanford University, Stanford, CA, United States of America
    \\
    * Corresponding author
    \\
    Email: andrewnam@stanford.edu (AN)
            
       
\end{titlepage}
